Scalable 3D Captioning with Pretrained Models

We introduce Cap3D, an automatic approach for generating descriptive text for 3D objects. This approach utilizes pretrained models from image captioning, image-text alignment, and LLM to consolidate captions from multiple views of a 3D asset, completely side-stepping the time-consuming and costly process of manual annotation. We apply Cap3D to the recently introduced large-scale 3D dataset, Objaverse, resulting in 660k 3D-text pairs. Our evaluation, conducted using 41k human annotations from the same dataset, demonstrates that Cap3D surpasses human-authored descriptions in terms of quality, cost, and speed. Through effective prompt engineering, Cap3D rivals human performance in generating geometric descriptions on 17k collected annotations from the ABO dataset. Finally, we finetune Text-to-3D models on Cap3D and human captions, and show Cap3D outperforms; and benchmark the SOTA including Point-E, Shape-E, and DreamFusion.

==> figures/ab_abo.tex <==
\begin{figure*}[t]
	\centering
			{\includegraphics[width=\linewidth]{figures/pdf/ab_abo.pdf}} % width=0.5\linewidth
	\caption{\textbf{ABO Caption A/B Evaluation.} We ask humans to select which caption best describes each object. Both Human and BLIP2 annotations significantly outperform Objaverse metadata; BLIP2 is usually better than Human captions.}
	\label{fig:ab_abo}
\end{figure*}


==> figures/ab_obja.tex <==
\begin{figure*}[t]
	\centering
			{\includegraphics[width=\linewidth]{figures/pdf/ab_obja.pdf}} % width=0.5\linewidth
	\caption{\textbf{Caption A/B Evaluation.} We ask humans to select which caption best describes each object. Both Human and BLIP2 annotations significantly outperform Objaverse metadata; BLIP2 is usually better than Human captions.}
	\label{fig:ab_obja}
\end{figure*}


==> figures/analysis_abo.tex <==
\begin{figure*}[t]
	\centering
			{\includegraphics[width=\linewidth]{figures/pdf/analysis_abo.pdf}} % width=0.5\linewidth
	\caption{\textbf{ABO Caption Statistics.} }
	\label{fig:analysis_abo}
\end{figure*}


==> figures/analysis_obja.tex <==
\begin{figure*}[t]
	\centering
			{\includegraphics[width=\linewidth]{figures/pdf/analysis_obja.pdf}} % width=0.5\linewidth
	\caption{\textbf{Objaverse Caption Statistics.} Human captions and internet metadata frequently have very short captions, while having a long tail of very long captions. Automatically generated captions are a consistent length.}
	\label{fig:analysis_obja}
\end{figure*}


==> figures/obja_caps.tex <==
\begin{figure*}[t]
	\centering
		{\includegraphics[width=\linewidth]{figures/pdf/obja_caps.pdf}} % width=0.5\linewidth
	\caption{\textbf{Objaverse Caption Comparison.} Human captions and Internet metadata frequently have very short captions, while having a long tail of very long captions. Automatically generated captions are a consistent length.}
	\label{fig:obja_caps}
\end{figure*}


==> figures/old/t23d_abo.tex <==
\begin{figure*}[t]
	\centering
			{\includegraphics[width=\linewidth]{figures/pdf/t23d_abo.pdf}} % width=0.5\linewidth
	\caption{\textbf{Text to 3D Generation.} .}
	\label{fig:t23d_abo}
\end{figure*}


==> tables/caption_abo_wrapped.tex <==
\begin{wraptable}{r}{7cm}
  \caption{\textbf{ABO Fine-Grained Geometry Captions}. Cap3D (QA) performs best; crowdsourced beats captioning alone.}
    \label{tab:caption_abo}
    \resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}{
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{Method} & A/B & A/B & A/B \\ 
     & Score (1-5) & Win \% & Lose \% \\
    \midrule
    Human v. Cap3D & 3.09$\pm$0.02 & 47.3$\pm$1\% & 41.4$\pm$1\% \\
    Cap3D(QA) v. Human & 3.08$\pm$0.02 & 50.2$\pm$1\% & 44.0$\pm$1\% \\
    Cap3D(QA) v. Cap3D & 3.27$\pm$0.02 & 56.0$\pm$1\% & 37.4$\pm$1\% \\
    Cap3D(QA) v. Meta & 4.27$\pm$0.02 & 88.2$\pm$1\% & 10.0$\pm$1\% \\
    %Human vs. Cap3D & 3.09\pm0.017 & 47.3\%\pm0.7\% & 47.3\%\pm0.7\% \\
    %Cap3D (QA) vs. Human & 3.08\pm0.020 & 50.2\%\pm0.7\% & 44.0\%\pm0.7\% \\
    %Cap3D (QA) vs. Cap3D & 3.27\pm 0.022 & 56.0\%\pm 0.8\% & 37.4\%\pm0.8\% \\
    %Cap3D (QA) vs. Meta & 4.27\pm 0.018 & 88.2\%\pm 0.6\% & 10.0\%\pm 0.6\% \\
    \bottomrule
    \end{tabular}
    }
\end{wraptable}


==> tables/old_unused/caption_abo.tex <==
\begin{table}
\caption{\textbf{ABO Fine-Grained Geometry Captions}. Crowdsourced annotation outperforms automated captioning in describing geometry. Given prompting, automated question answering (QA) performs best.}
\label{tab:caption_abo}
\resizebox{\ifdim\width>0.5\linewidth 0.5\linewidth \else \width \fi}{!}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Method} & A/B & A/B & A/B \\ 
 & Score (1-5) & Win \% & Lose \% \\
\midrule
Human vs. Ours & 3.09$\pm$0.02 & 47.3$\pm$1\% & 41.4$\pm$1\% \\
Ours (QA) vs. Human & 3.08$\pm$0.02 & 50.2$\pm$1\% & 44.0$\pm$1\% \\
Ours (QA) vs. Ours & 3.27$\pm$0.02 & 56.0$\pm$1\% & 37.4$\pm$1\% \\
Ours (QA) vs. Meta & 4.27$\pm$0.02 & 88.2$\pm$1\% & 10.0$\pm$1\% \\
%Human vs. Ours & 3.09\pm0.017 & 47.3\%\pm0.7\% & 47.3\%\pm0.7\% \\
%Ours (QA) vs. Human & 3.08\pm0.020 & 50.2\%\pm0.7\% & 44.0\%\pm0.7\% \\
%Ours (QA) vs. Ours & 3.27\pm 0.022 & 56.0\%\pm 0.8\% & 37.4\%\pm0.8\% \\
%Ours (QA) vs. Meta & 4.27\pm 0.018 & 88.2\%\pm 0.6\% & 10.0\%\pm 0.6\% \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/clip_full_dset.tex <==
\begin{table}
\caption{\textbf{Caption Quality on Full Dataset}. .}
\label{tab:clip_full_dset}
\resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{4}{c}{Objaverse} \\
\multirow{2}{*}{Method} & CLIP & ViLBERT & \multirow{2}{*}{TIGER} \\ 
 & Score & Score-F & \\
\midrule
Objaverse & & & & \\
BLIP2 & & & & \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/old_text_3d_300obj.tex <==
\begin{table}
\caption{\textbf{Text-3D: Optimization Baselines}. .}
\label{tab:text_3d}
\resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}{
\begin{tabular}{lccccc}
\toprule
& \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (300)} \\
& & Score & R@1 & R@5 & R@10 \\
\midrule
Ground Truth Images & - & 83.2 & 53.2 & 77.8 & 86.9 \\
\midrule
Shape Compiler & 288.7 & 56.4 &	0.2 & 1.7 &	3.7  \\ 
DreamField & 106.1 & 83.7 &	61.8 & 83.6 & 91.2 \\ 
Stable DreamFusion & 127.8 & 72.4 & 28.4 & 46.1 & 55.2\\ 
3D Fuse & 93.4 & 75.8 & 38.8 & 59.5	& 66.8  \\ 
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/text_3d_300obj.tex <==
\begin{table}
\caption{\textbf{Text-3D: Optimization Baselines}. Overfitting via CLIP leads to higher scores than ground truth; ViLT score is more fair.}
\label{tab:text_3d_300obj}
\resizebox{\ifdim\width>0.5\linewidth 0.5\linewidth \else \width \fi}{!}{
\begin{tabular}{lcccccc}
\toprule
%& \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (300)} \\
& \multirow{2}{*}{FID$\downarrow$} & \multicolumn{3}{c}{CLIP} & \multicolumn{2}{c}{ViLT} \\
& & Score & R@1 & R@5 & R@1 & R@5 \\
\midrule
Ground Truth Images & - & 83.2 & 53.2 & 77.8 & 41.3 & 69.0 \\
\midrule
Shape Compiler~\cite{luo2023neural} & 288.7 & 56.4 &	0.2 & 1.7 &	0.3 & 1.0 \\ 
DreamField~\cite{jain2022zero} & 106.1 & \textbf{83.7} &	\textbf{61.8} & \textbf{83.6} & \textbf{32.3} & \textbf{56.0} \\ 
Stable DreamFusion~\cite{poole2022dreamfusion} & 127.8 & 72.4 & 28.4 & 46.1 & 23.7 & 45.3 \\ 
3D Fuse~\cite{seo2023let} & \textbf{93.4} & 75.8 & 38.8 & 59.5	& 24.7 & 51.0 \\ 
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/text_3d_obja_full.tex <==
\begin{table}
\caption{\textbf{Text to 3D on Objaverse}. .}
\label{tab:text_3d_obja}
\resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}{
\begin{tabular}{lcccccccccccccccccc}
\toprule
& \multicolumn{8}{c}{Pretrained} & \multicolumn{8}{c}{Finetuned on Ours} \\
%& \multirow{3}{*}{FID} & & & & \multirow{3}{*}{FID} & & \\
%& & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k) & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k) & & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k) & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
& \multirow{3}{*}{FID} & \multicolumn{4}{c}{ViT-B/32} & \multicolumn{4}{c}{ViT-L/14} & \multirow{3}{*}{FID} & \multicolumn{4}{c}{ViT-B/32} & \multicolumn{4}{c}{ViT-L/14} \\
& & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k)} & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k)} & & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k)} & \multirow{2}{*}{CLIP Score} & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
& & & R@1 & R@5 & R@10 & & R@1 & R@5 & R@10 & & R@1 & R@5 & R@10 & & R@1 & R@5 & R@10 \\
\midrule
Ground Truth Images \\
\midrule
Point-E (Text-3D) &&& &\\ 
Stable Diffusion (CtrlNet) + Point-E (Img-3D)  &&& &\\ 
Stable Diffusion (LoRA) + Point-E (Img-3D)  & & & & \\
ShapE t23D (STF) & & & & \\
ShapE (NeRF) & & & & \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/text_3d_vs_human.tex <==
\begin{table}
\caption{\textbf{Text-3D: Human Captions}. Finetuning improves Point·E performance. On the small set, our captions are better than human; the full dataset improves further. Finetuning Shap·E does not improve regardless of data or method; the smallest decline is upon Full Set (Ours).}
\label{tab:text_3d_vs_human}
\resizebox{\ifdim\width>0.5\linewidth 0.5\linewidth \else \width \fi}{!}{
\begin{tabular}{clccccc}
\toprule
& \multirow{2}{*}{Finetune Dataset} & \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
& & & Score & R@1 & R@5 & R@10 \\
%\midrule
%Ground Truth Images & - & 81.6 & 32.7 &	55.1 & 64.3 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Point·E}} & Pretrained Only & 36.1 & 72.4 & 6.0	& 16.2 & 22.4 \\ %(Text-3D)~\cite{nichol2022point} ~\cite{nichol2022point}: 
& Small Set (Human) & 34.6 & 74.4 & 8.2 & 21.3 & 29.1 \\
& Small Set (Ours) & \underline{33.7} & \underline{75.0} & \underline{10.4} & \underline{24.3} & \underline{32.1} \\ 
& Full Set (Ours) & \textbf{32.8} & \textbf{75.6} & \textbf{12.4} & \textbf{28.1} & \textbf{36.9} \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Shap·E}} & Pretrained Only & 37.2 & \textbf{80.4} & \textbf{20.3} & \textbf{39.7} &	\textbf{48.7} \\ %(STF)~\cite{gao2022get3d}: 
& Small Set (Human) & \underline{36.0} & \underline{79.6} & 18.6 & 36.3 & 45.3 \\
& Small Set (Ours) & 37.2 & 79.4 & 19.1 & 37.5 & 46.1 \\
& Full Set (Ours) & \textbf{35.5} & 79.1 & \underline{20.0} & \underline{38.8} & \underline{47.3} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/text_3d_vs_human_old.tex <==
\begin{table}
\caption{\textbf{Text to 3D on Objaverse}. .}
\label{tab:text_3d_obja}
\resizebox{\ifdim\width>0.5\linewidth 0.5\linewidth \else \width \fi}{!}{
\begin{tabular}{cclccccc}
\toprule
& & \multirow{2}{*}{Finetune Dataset} & \multirow{2}{*}{FID} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
& & & & Score & R@1 & R@5 & R@10 \\
%\midrule
%Ground Truth Images & - & 81.6 & 32.7 &	55.1 & 64.3 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Point-E}} & \multirow{4}{*}{\rotatebox{90}{(Text-3D)}} & Pretrained Only & 36.1 & 72.4 & 6.0	& 16.2 & 22.4 \\ %(Text-3D)~\cite{nichol2022point} ~\cite{nichol2022point}: 
& & Small Set (Human) & 34.6 & 74.4 & 8.2 & 21.3 & 29.1 \\
& & Small Set (Ours) & 33.7	& 75.0 & 10.4 & 24.3 & 32.1 \\ 
& & Full Set (Ours) & 32.8 & 75.6 &	12.4 & 28.1 & 36.9 \\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Shap-E}} & \multirow{4}{*}{\rotatebox{90}{(STF)}} & Pretrained Only & 37.2 & 80.4 & 20.3 & 39.7 &	48.7 \\ %(STF)~\cite{gao2022get3d}: 
& & Small Set (Human) & 36.0 & 79.6 & 18.6 & 36.3 & 45.3 \\
& & Small Set (Ours) & 37.2 & 79.4 & 19.1 & 37.5 & 46.1 \\
& & Full Set (Ours) & 35.5 & 79.1 & 20.0 & 38.8 & 47.3 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/old_unused/text_3d_vs_human_wrapped.tex <==
\begin{wraptable}{r}{7cm}
  \caption{\textbf{Text-3D: Human Captions}. Finetuning improves Point·E performance. On the small set, our captions are better than human; the full dataset improves further. Finetuning Shap·E does not improve regardless of data or method; the smallest decline is upon Full Set (Ours).}
  \label{tab:text_3d_vs_human_wrapped}
  \resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}
  {
    \begin{tabular}{clccccc}
    \toprule
    & \multirow{2}{*}{Finetune Dataset} & \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
    & & & Score & R@1 & R@5 & R@10 \\
    %\midrule
    %Ground Truth Images & - & 81.6 & 32.7 &	55.1 & 64.3 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Point·E}} & Pretrained Only & 36.1 & 72.4 & 6.0	& 16.2 & 22.4 \\ %(Text-3D)~\cite{nichol2022point} ~\cite{nichol2022point}: 
    & Small Set (Human) & 34.6 & 74.4 & 8.2 & 21.3 & 29.1 \\
    & Small Set (Ours) & \underline{33.7} & \underline{75.0} & \underline{10.4} & \underline{24.3} & \underline{32.1} \\ 
    & Full Set (Ours) & \textbf{32.8} & \textbf{75.6} & \textbf{12.4} & \textbf{28.1} & \textbf{36.9} \\ 
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Shap·E}} & Pretrained Only & 37.2 & \textbf{80.4} & \textbf{20.3} & \textbf{39.7} &	\textbf{48.7} \\ %(STF)~\cite{gao2022get3d}: 
    & Small Set (Human) & \underline{36.0} & \underline{79.6} & 18.6 & 36.3 & 45.3 \\
    & Small Set (Ours) & 37.2 & 79.4 & 19.1 & 37.5 & 46.1 \\
    & Full Set (Ours) & \textbf{35.5} & 79.1 & \underline{20.0} & \underline{38.8} & \underline{47.3} \\
    \bottomrule
    \end{tabular}
    }
\end{wraptable}


==> tables/text_3d_300obj_vs_human.tex <==
\begin{table}[t]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \captionsetup{width=0.95\textwidth}
  \caption{\textbf{Text-3D: Optimization Baselines}. Overfitting via CLIP leads to higher scores than ground truth; ViLT score is more fair.}
  \resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}
    {
    \begin{tabular}{lcccccc}
    \toprule
    %& \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (300)} \\
    & \multirow{2}{*}{FID$\downarrow$} & \multicolumn{3}{c}{CLIP} & \multicolumn{2}{c}{ViLT} \\
    & & Score & R@1 & R@5 & R@1 & R@5 \\
    \midrule
    True Images & - & 83.2 & 53.2 & 77.8 & 41.3 & 69.0 \\
    \midrule
    NSC~\cite{luo2023neural} & 288.7 & 56.4 &	0.2 & 1.7 &	0.3 & 1.0 \\ 
    D. Field~\cite{jain2022zero} & 106.1 & \textbf{83.7} &	\textbf{61.8} & \textbf{83.6} & \textbf{32.3} & \textbf{56.0} \\ 
    D. Fusion~\cite{poole2022dreamfusion} & 125.9 & 73.2 & 29.7 & 48.3 &  & 24.7 & 47.7 \\ 
    3DFuse~\cite{seo2023let} & \textbf{91.1} & 77.0 & 38.6 & 58.5 & 26.3 & 53.0 \\ 
    %D. Fusion~\cite{poole2022dreamfusion} & 127.8 & 72.4 & 28.4 & 46.1 & 23.7 & 45.3 \\ 
    %3DFuse~\cite{seo2023let} & \textbf{93.4} & 75.8 & 38.8 & 59.5	& 24.7 & 51.0 \\ 
    \bottomrule
    \end{tabular}
    }
  \label{tab:table1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \captionsetup{width=0.95\textwidth}
  %\caption{\textbf{Text-3D: Human Captions}. Finetuning improves Point·E performance. On the small set, our captions are better than human; the full dataset improves further. Finetuning Shap·E does not improve regardless of data or method; the smallest decline is upon Full Set (Ours).}
  \caption{\textbf{Text-3D: Human Captions}. Our captions are better than human on the 30k set.}
  \resizebox{\ifdim\width>\linewidth \linewidth \else \width \fi}{!}
    {
    \begin{tabular}{clccccc}
    \toprule
    & Finetune & \multirow{2}{*}{FID$\downarrow$} & CLIP  & \multicolumn{3}{c}{CLIP R-Precision (2k)} \\
    & Dataset & & Score & R@1 & R@5 & R@10 \\
    %\midrule
    %Ground Truth Images & - & 81.6 & 32.7 &	55.1 & 64.3 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Point·E}} & Pretrained & 36.1 & 72.4 & 6.0	& 16.2 & 22.4 \\ %(Text-3D)~\cite{nichol2022point} ~\cite{nichol2022point}: 
    & 30k (Human) & 34.6 & 74.4 & 8.2 & 21.3 & 29.1 \\
    & 30k (Ours) & \underline{33.7} & \underline{75.0} & \underline{10.4} & \underline{24.3} & \underline{32.1} \\ 
    & Full (Ours) & \textbf{32.8} & \textbf{75.6} & \textbf{12.4} & \textbf{28.1} & \textbf{36.9} \\ 
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Shap·E}} & Pretrained & 37.2 & \textbf{80.4} & \textbf{20.3} & \textbf{39.7} &	\textbf{48.7} \\ %(STF)~\cite{gao2022get3d}: 
    & 30k (Human) & \underline{36.0} & \underline{79.6} & 18.6 & 36.3 & 45.3 \\
    & 30k (Ours) & 37.2 & 79.4 & 19.1 & 37.5 & 46.1 \\
    & Full (Ours) & \textbf{35.5} & 79.1 & \underline{20.0} & \underline{38.8} & \underline{47.3} \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:table2}
\end{minipage}
\end{table}

